Dynamic Graph Communication for Decentralised Multi-Agent Reinforcement Learning

This work presents a novel communication framework for decentralized multi-agent systems operating in dynamic network environments. Integrated into a multi-agent reinforcement learning system, the framework is designed to enhance decision-making by optimizing the network's collective knowledge through efficient communication. Key contributions include adapting a static network packet-routing scenario to a dynamic setting with node failures, incorporating a graph attention network layer in a recurrent message-passing framework, and introducing a multi-round communication targeting mechanism. This approach enables an attention-based aggregation mechanism to be successfully trained within a sparse-reward, dynamic network packet-routing environment using only reinforcement learning. Experimental results show improvements in routing performance, including a 9.5 percent increase in average rewards and a 6.4 percent reduction in communication overhead compared to a baseline system. The study also examines the ethical and legal implications of deploying such systems in critical infrastructure and military contexts, identifies current limitations, and suggests potential directions for future research.

==> sections/2.background_and_literature_review.tex <==
% \section{Reinforcement Learning}
% \label{sec:reinforcement-learning}

% The origins of reinforcement learning (RL) can be traced back to the research on animal behaviourism pioneered by B.F. Skinner, a key proponent of the behaviourist theory of learning. This theory suggests that learning is a process of conditioning an animal's behaviour within an environment of stimuli, rewards, and punishments \cite{skinner1938behavior}. Reinforcement learning builds on this concept by extending it to computational agents, enabling computers to emulate the learning processes observed in animals. This powerful mechanism has proven exceptionally effective in complex sequential decision-making tasks, achieving superhuman performance in both board games \cite{silver2016mastering, silver2017mastering} and computer games \cite{mnih2013playing}. Beyond gaming, reinforcement learning has also made significant strides in real-world applications, particularly in fields such as robotics \cite{kober2013reinforcement}, autonomous driving \cite{zhang2023high}, and natural language processing \cite{christiano2017deep}.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/agent-enviroment-interaction.png}
%     \caption{Agent-Environment interaction within a Markov Decision Process \cite{sutton2018reinforcement}: The agent receives the current state $s_t$ from the environment and takes an action $a_t$. The environment then provides a reward $r_t$ and the next state $s_{t+1}$.}
%     \label{fig:enter-label}
% \end{figure}

% The core of reinforcement learning is the interaction between an agent and its environment, The agent observes the current state of the environment and takes an action according to its learned policy (mapping of state to action). The environment then transitions to a new state and emits a scalar reward signal which reflects the consequences of the action taken. This is an iterative process, with the agent continuously learning how to improve its policy to maximize the cumulative reward over time \cite{sutton2018reinforcement}. 


% \subsubsection{Markov Decision Process}

% The environment in reinforcement learning is typically represented as an infinite-horizon discounted Markov Decision Process (MDP) \cite{bellman1957markovian}. An MDP provides a mathematical framework for representing stochastic sequential decision-making processes that exhibit the Markov property. This property implies that the future state of the process depends solely on the current state, independent of the sequence of events that led to it. According to the conditions specified by Puterman \cite{puterman2014markov}, an optimal policy for any given MDP is both deterministic and Markovian.

% \vspace{12pt}

% We can formally defined a MDP as a quintuple \( (S, A, R, P, \gamma) \).

% \begin{itemize}
%     \item \textbf{State Space \((S)\)}: A finite set of states, \(S\), representing all possible situations that could occur.
%     \item \textbf{Action Space \((A)\)}: For each state \(s\), there exists a finite set of actions \(A(s)\) available to the agent.
%     \item \textbf{Transition Probability \((P)\)}: The probability \(P(s_{t+1}|s_t,a_t)\) that action \(a_t\) in state \(s_t\) at time \(t\) will lead to state \(s_{t+1}\) at time \(t+1\).
%     \item \textbf{Reward Function \((R)\)}: A reward function \(R(s_t,a_t,s_{t+1})\) specifying the immediate reward received after transitioning from state \(s\) to state \(s_{t+1}\), due to action \(a_t\).
%     \item \textbf{Discount Factor \((\gamma)\)}: A factor \(\gamma \in [0, 1]\) that represents the difference in importance between future rewards and present rewards.
% \end{itemize}


% \subsection{Dynamic Programming}
% \label{sec: dynamic programming}

% The objective of a reinforcement learning agent is to determine the optimal policy \( \pi^* \) that maximizes the expected cumulative reward. The conventional approach to this problem involves computing the optimal value function \( V^*(s) \) for each state \( s \), which in turn informs a greedy policy that selects actions maximizing the expected value of the next state. Using the Markovian assumption, we can decompose the value of each state \( V^\pi(s) \) into the expected immediate reward received \( R(s,a) \) and the expected discounted value of the successor states \( \gamma V^\pi(s') \), where \( s' \) represents the next state.

% \begin{equation}
% V^\pi(s) = \mathbb{E}_\pi[R_t \mid S_t = s] = \sum_{a} \pi(s, a) \sum_{s'} P^a_{ss'} \left[ R^a_{ss'} + \gamma V^\pi(s') \right]
% \end{equation}

% In practice, it is often more effective to calculate the action values \( Q^*(s, a) \), which represent the value of taking a specific action \( a \) in a state \( s \). The action-value function for policy \( \pi \) is given by:

% \begin{equation}
% Q^\pi(s, a) = \mathbb{E}_\pi[R_t \mid S_t = s, A_t = a] = \sum_{s'} P^a_{ss'} \left[ R^a_{ss'} + \gamma \sum_{a'} \pi(s', a') Q^\pi(s', a') \right]
% \end{equation}

% By decomposing the value functions, the problem is formulated as a series of overlapping subproblems. Bellman proposed solving them recursively using dynamic programming to determine the optimal state value function \( V^*(s) \) and the optimal action value function \( Q^*(s, a) \), leading to the \textit{Bellman Optimality Equations (BOE)} for both \cite{bellman1957markovian}:

% \begin{equation}
% \label{eq: bellman}
% V^*(s) = \max_a \sum_{s'} P^a_{ss'} \left[ R^a_{ss'} + \gamma V^*(s') \right] 
% \end{equation}

% \begin{equation}
% Q^*(s, a) = \sum_{s'} P^a_{ss'} \left[ R^a_{ss'} + \gamma \max_{a'} Q^*(s', a') \right]
% \end{equation}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/backup_diagrams.png}
%     \caption{Backup diagrams for solving Bellman Optimality Equations recursively: (a) optimal state value function \( V^*(s) \) (b) optimal action value function \( Q^*(s, a) \) \cite{sutton2018reinforcement}}
%     \label{fig:enter-label}
% \end{figure}

% Dynamic programming techniques, such as \textit{Value Iteration} and \textit{Policy Iteration}, can be employed to solve the MDP by iteratively approximating the optimal policy. These methods assume complete knowledge of the MDP's dynamics and are guaranteed to converge to the optimal policy under conditions such as finite state and action spaces, and the requirement that all states or state-action pairs are visited infinitely often \cite{sutton2018reinforcement}. The optimal policy can be derived from the optimal action-value function using a greedy deterministic approach:

% \begin{equation}
% \pi^* = \arg\max_a Q^*(s, a), \quad \forall s \in S, \forall a \in A
% \end{equation}

% \subsubsection{Monte Carlo Learning}

% Dynamic programming techniques rely on complete knowledge of the environment's dynamics to directly calculate values of states and state-actions, including transition probabilities and reward functions. Methods that leverage this knowledge or attempt to learn the environment's dynamics are referred to as \textit{model-based} methods. However, in many environments, the dynamics are either inaccessible or too complex to model accurately. 

% \vspace{12pt}

% An alternative approach is to estimate these values based on accumulated experience, known as \textit{model-free} methods. \textit{Monte Carlo (MC)} methods, such as MCTS \cite{coulom2006efficient}, approach this problem by sampling trajectories through the environment, collating the returns received when visiting each state, and finally, at the end of a full episode, calculating the average reward received for each state or state action. The MC value estimation equation is:

% \begin{equation}
% V(s) = \frac{1}{N} \sum_{i=1}^{N} G_i(s)
% \end{equation}

% where \( V(s) \) is the value of state \( s \), \( N \) is the number of episodes in which state \( s \) is visited, and \( G_i(s) \) is the return (cumulative reward) following the \( i \)-th visit to state \( s \).

% \subsubsection{Temporal Difference Learning}

% While Monte Carlo methods provide unbiased value estimates, they require complete episodes for updates, limiting their applicability in non-episodic environments. \textit{Temporal Difference (TD)} learning \cite{sutton1988learning} methods address this limitation by allowing value updates from incomplete episodes through \textit{bootstrapping} value estimates of subsequent states. 

% \vspace{12pt}

% TD learning combines ideas from both Monte Carlo methods and dynamic programming, providing a more general framework. The basic Temporal Difference error for TD(0), which updates value estimates based on the reward received and the estimated value of the subsequent state, is given by the equation:

% \begin{equation}
%     \delta_t = R_{t+1} + \gamma V(s_{t+1}) - V(s_t)
% \end{equation}

% where \( \delta_t \) is the TD error, \( R_{t+1} \) is the reward after taking action \( a_t \) in state \( s_t \), \( \gamma \) is the discount factor, and \( V(s) \) represents the value of a state. The advantage of TD is that updating from incomplete experience generally results in faster, more stable convergence. However, using bootstrapped estimates of subsequent states introduces a bias.

% \subsection{Value Based Reinforcement Learning}

% Methods that utilize intermediate value functions, such as TD Learning , for policy optimization are known as \textit{value-based methods}. TD learning is an \textit{on-policy} algorithm, meaning it learns the value of the policy being followed by the agent through its own exploration. This approach allows the agent to improve its policy based on the values of the states it actually visits.

% \subsubsection{Q-Learning}

% In contrast, \textit{Q-learning} \cite{watkins1989learning}, introduced by Watkins in 1989, extends TD learning by being an \textit{off-policy} algorithm. This means Q-learning can learn the value of the optimal policy regardless of the agent's actions. It accomplishes this by evaluating the best possible action at each state, rather than only the actions taken by the agent, providing greater flexibility and robustness in learning the optimal policy. The Q-learning update rule is given by:

% \begin{equation}
% Q(s, a) \leftarrow Q(s, a) + \alpha \left[ r + \gamma \max_{a'} Q(s', a') - Q(s, a) \right]
% \end{equation}

% \subsubsection{Deep Q-Network}

% Traditional tabular reinforcement learning methods, such as Q-learning, face significant challenges in handling large state and action spaces due to their high memory and computational demands. As these spaces grow, tabular approaches become inefficient and struggle to generalize to unseen states.

% \vspace{12pt}

% \textit{Deep Q-Networks} (DQNs) \cite{mnih2013playing} address these limitations by leveraging neural networks to approximate the Q-value function, eliminating the need for a lookup table. This enables DQNs to effectively manage large and continuous state spaces, making them suitable for complex and high-dimensional problems.

% \begin{figure}[H]
%     \centering
%     \hspace*{-0.2\linewidth} % Adjust this value as needed to move the image left
%     \includegraphics[width=0.75\linewidth]{figures/DQN-structure.png}
%     \caption{Deep Q-Network (DQN) Architecture \cite{cong2021deep}: The agent utilizes memory replay to store and sample experiences for training. The Q-network is trained by minimizing the loss between the predicted Q value and the target Q value, with periodic updates to the target network's weights ($\theta \rightarrow \theta'$).}
%     \label{fig:DQN}
% \end{figure}

% \addvspace{12pt}

% DQNs achieve off-policy learning through the use of two separate networks: the \textit{behavior network}, which selects actions, and the \textit{target network}, which generates the target Q-values. The target network is a periodically updated copy of the behavior network, providing more stable targets for learning and helping to mitigate the risk of feedback loops that can destabilize training. Additionally, DQNs incorporate an \textit{experience replay buffer} to store past experiences and randomly sample them during training. This technique improves sampling efficiency, reduces the correlation between consecutive experiences, and further stabilizes the learning process.

% \subsection{Policy Based Reinforcement Learning}

% Value-based methods determine the optimal policy by using the \(\text{argmax}\) function over state values, but this approach confines them to discrete action spaces. To overcome this limitation, \textit{policy-based methods} conduct a direct search within the policy space, bypassing the need for intermediate value functions and permitting use within continuous action spaces. These methods are based on the \textit{Policy Gradient (PG) Theorem} introduced by Sutton \cite{sutton1999policy}, which provides a method for computing the gradient of the expected return with respect to the policy parameters \(\theta\).

% \begin{gather}
% \label{eq: PG}
% \nabla_{\theta} J(\pi_{\theta}) = \mathbb{E}_{\tau \sim \pi_{\theta}} \left[ \sum_{t=0}^{T} \nabla_{\theta} \log \pi_{\theta}(a_t \mid s_t) \cdot Q^{\pi_{\theta}}(s_t, a_t) \right] \\
% \theta_{new} = \theta_{old} + \alpha \nabla_{\theta} J(\pi_{\theta})
% \end{gather}

% Here, \( \tau = (s_0, a_0, s_1, a_1, \ldots, s_T, a_T) \) represents a trajectory that follows the policy \( \pi_{\theta} \), where \( T \) denotes the time horizon. \( Q^{\pi_{\theta}}(s_t, a_t) \) is the action value function under the policy \( \pi_{\theta} \), and \( \alpha \) represents the learning rate.

% \vspace{12pt}

% Beyond their applicability to continuous action spaces, policy-based methods offer several additional advantages over value-based methods. Firstly, by directly parameterizing the policy, these methods are more effective in handling high-dimensional action spaces. Secondly, their direct optimization of the policy typically results in superior convergence properties. Lastly, policy-based methods can learn stochastic policies, which are particularly beneficial in environments with inherent uncertainty or where a diverse set of actions is advantageous.

% \subsubsection{REINFORCE}

% The foundational policy-based algorithms are \textit{REINFORCE} \cite{williams1992simple}, a Monte Carlo PG method that uses episodic returns to update the policy parameters. The update rule for REINFORCE is given by:

% \begin{equation}
%     \theta_{new} = \theta_{old} + \alpha \sum_{t=0}^{T} \nabla_{\theta} \log \pi_{\theta}(a_t \mid s_t) \cdot G_t
% \end{equation}

% Here, \( G_t \) represents the return (cumulative reward) from time step \( t \) onward. The gradient \( \nabla_{\theta} \log \pi_{\theta}(a_t \mid s_t) \) indicates how to adjust the policy parameters to increase the likelihood of actions that lead to higher returns.

% \subsection{Actor-Critic Reinforcement Learning}

% Policy-based methods offer several advantages but are often hindered by high variance in gradient estimates, especially in environments with sparse rewards. Actor-Critic methods \cite{barto1983neuronlike, konda1999actor} address this issue by introducing a \textit{critic} network that estimates the value function. This reduces the variance in the feedback used for the \textit{actor} network's policy gradient updates, resulting in more stable and efficient learning.

% \addvspace{12pt}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/actor-critic.png}
%     \caption{Actor-Critic Framework: The Actor (Policy) selects actions based on the state. The Critic (Value Function) evaluates these actions using the TD error to update both the Policy and Value Function, iteratively improving performance.}
%     \label{fig:actor-critic-framework}
% \end{figure}

% \addvspace{12pt}

% This hybrid framework leverages the strengths of both policy-based (actor) and value-based (critic) methods by employing two separate components, typically implemented with individual neural networks:

% \begin{itemize}
% \item \textbf{Actor:} Proposes actions based on a policy and updates the policy parameters using policy gradient methods.
% \item \textbf{Critic:} Evaluates the actions proposed by the actor and provides feedback using value-based methods, such as Temporal Difference learning.
% \end{itemize}

% By decoupling policy and value estimations, Actor-Critic methods often achieve faster convergence. This separation allows the actor to focus directly on maximizing rewards, while the critic provides grounded value estimates that help reduce variance in policy updates. The dual approach also permits different learning rates for the actor and critic, optimizing learning efficiency and stability.

% \subsubsection{Proximal Policy Optimization}

% \textit{Proximal Policy Optimization (PPO)} \cite{schulman2017proximal} is a state-of-the-art actor-critic algorithm introduced by Schulman et al., which constrains policy updates to a small region to prevent large, destabilizing updates that can lead to poor performance. PPO achieves this by using a surrogate objective function that includes a penalty for deviating too far from the previous policy. This can be expressed as:

% \begin{equation}
% \label{eq:ippo-loss}
%     L^{CLIP}(\theta) = \mathbb{E}_{t} \left[ \min \left( r_t(\theta) \hat{A}_t, \text{clip}(r_t(\theta), 1 - \epsilon, 1 + \epsilon) \hat{A}_t \right) \right]
% \end{equation}

% where \( r_t(\theta) = \frac{\pi_{\theta}(a_t \mid s_t)}{\pi_{\theta_{old}}(a_t \mid s_t)} \) is the probability ratio, \( \hat{A}_t \) is the advantage estimate, and \( \epsilon \) is a small hyperparameter that controls the clipping range.

% \vspace{12pt}

% To calculate the advantage estimate \( \hat{A}_t \), PPO leverages \textit{Generalized Advantage Estimation (GAE)}. The traditional advantage function \( A^{\pi}(s_t, a_t) = Q^{\pi}(s_t, a_t) - V^{\pi}(s_t) \), commonly used in critic networks to increase stability, measures the benefit of taking action \( a \) in state \( s \) compared to the average action. Introduced by Schulman et al. \cite{schulman2015high}, GAE refines this advantage function by considering multiple future steps, which reduces the variance of the estimates at the cost of increased bias. This bias-variance trade-off is controlled by a parameter \( \lambda \), which adjusts the weighting of future steps. GAE uses the TD error, defined as \( \delta_t = R_t + \gamma V(s_{t+1}) - V(s_t) \), to calculate the advantage estimate:

% \begin{equation}
%     A_t^{GAE(\gamma, \lambda)} = \sum_{l=0}^{\infty} (\gamma \lambda)^l \delta_{t+l}
% \end{equation}


% \subsubsection{Deep Deterministic Policy Gradient}

% \textit{Deep Deterministic Policy Gradient (DDPG)} \cite{lillicrap2015continuous}, introduced by Lillicrap et al., is a state-of-the-art actor-critic algorithm designed for continuous action spaces. DDPG uses a deterministic policy, \(\mu_{\theta}(a|s)\), which simplifies the exploration-exploitation trade-off by directly mapping states to specific actions, reducing the complexity of exploring continuous action spaces. As an off-policy algorithm, DDPG also employs experience replay and target networks to further stabilize training. The deterministic policy gradient update in DDPG is given below:

% \begin{align}
% \nabla_{\theta}J(\theta) = \mathbb{E}_{s}[\nabla_{\theta}\mu_{\theta}(a|s)\nabla_{a}Q^{\mu}(s, a)],
% \label{eq:DPG}
% \end{align}

% \section{Multi-Agent Systems}

% As intelligent and autonomous systems become more prevalent, effectively managing interactions between multiple autonomous agents has become increasingly important. Multi-Agent Systems (MAS), which involve multiple agents operating within a shared environment, play a crucial role in a variety of domains, including robotics \cite{yu2023asynchronous}, autonomous vehicles \cite{kiran2021deep}, and financial markets \cite{shavandi2022multi}. These systems enable agents to cooperate, compete, and coordinate their actions to achieve complex goals unattainable by a single agent.

% \subsection{Challenges in a Multi-Agent System}

% The dynamic and interactive nature of multi-agent systems introduces unique challenges not encountered in single-agent systems. These challenges stem from the complexities of coordinating and learning in an environment influenced by multiple agents, each with their own objectives and behaviors. Key challenges include partial observability, non-stationarity, credit assignment and scalability.

% \subsubsection{Partial Observability}

% In a MDP, it is assumed that agents can fully observe the global state of the environment. However, in many real-world applications, agents must make decisions based on incomplete information due to factors such as scale, privacy, or communication constraints.

% \vspace{12pt}

% To extend the single agent MDP to a partially observable environment, forming a \textit{Partially Observable MDP (POMDP)}, we introduce the concept of observations \( o_t \). At timestep \( t \), the environment is in state \( s_t \) and emits an observation \( o_t \) specific to the agent from the space of possible observations \( O \). The agent receives this observation and uses it to update its internal belief state \( b_t \) using Bayes' rule. The belief state represents the agent's probability distribution over the current state based on received observations. The agent then selects an action \( a_{t+1} \) based on \( b_{t+1} \) using the policy function \( \pi(b_{t+1}) \).

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/pompd.png}
%     \caption{POMDP framework: The agent updates its belief state \( b_t \) based on observations \( o_t \) and selects actions \( a_{t+1} \) according to its policy. The environment transitions to a new state \( s_{t+1} \), emits an observation, and provides a reward \( r_t \).}
%     \label{fig:pompd}
% \end{figure}

% Partial observability complicates the decision-making process by forcing the agent to rely on its belief state to infer hidden aspects of the environment, which in turn reduces sample efficiency as the agent needs to accumulate more experiences to accurately map observations to potential current states \cite{du2023review}. Consequently, the computational complexity of solving POMDPs is increased from P-Class (MDP) to PSPACE-complete, making it a highly challenging problem \cite{mundhenk2000complexity}.

% \subsubsection{Non-Stationarity}

% In single-agent environments, dynamics are typically stationary, with consistent transition probabilities and reward functions for state-action pairs. However, in multi-agent systems, the outcome (next state and reward) for an agent depends on the joint actions of all agents. This interdependence creates a non-stationary environment for each agent, as the current state no longer fully represents all relevant information. This breaks the Markovian assumption, invalidates traditional Q-learning convergence guarantees \cite{hernandez2017survey}, and introduces increased variance in the learning process.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/non-stationary-enviroment.png}
% \caption{A non-stationary environment in a multi-agent system, where each "model" represents an agent. Agents' actions \(a_t\) cause transitions between states \(S_1, S_2, S_3\), with evolving system dynamics as agents update their policies.}
% \label{fig}
% \end{figure}


% Non-stationarity increases learning variance and makes it difficult for agents to converge on optimal policies. The ever-changing dynamics due to policy updates require agents to constantly adapt, leading to instability and slower learning, necessitating more advanced techniques to handle the complexity.

% \subsubsection{Credit Assignment}

% In single-agent RL, the process of distributing rewards across past actions is known as \textit{temporal credit assignment} or \textit{reward redistribution} \cite{sutton2018reinforcement}. This challenge becomes more complex in multi-agent systems, where multiple agents contribute to a shared outcome. Identifying each agent's contribution to the collective performance is difficult, particularly in cooperative tasks with a joint reward signal. Even with centralized control, ineffective reward distribution in partially observable environments can hinder cooperation and lead to the \textit{lazy agent} phenomenon \cite{sunehag2017value}, where agents are disincentivized from exploring to avoid disrupting the effective policies of others.

% \subsubsection{Scalability}

% As the number of agents in a system grows, the information that needs to be shared and processed increases exponentially. This \textit{combinatorial nature} of Multi-Agent Reinforcement Learning refers to the exponential growth in the joint action space with more agents \cite{hernandez2019survey}, making centralized control computationally infeasible. To address this, decentralized and hierarchical control structures are often employed. Decentralized approaches distribute the computational load, enabling agents to make decisions based on local information with limited communication. Hierarchical structures break the problem into smaller sub-problems, organizing agents into layers with distinct decision-making roles.

% \subsection{Interaction Types in a Multi-Agent System}

% Multi-agent systems are primarily categorized by the type of interactions among agents. Understanding how individual agent objectives align or diverge from collective goals is essential for effectively shaping and distributing rewards.

% \vspace{12pt}

% In the Markov games framework, the optimal solution for a multi-agent system is often an equilibrium point known as the \textit{Nash Equilibrium (NE)} \cite{nash1950non, bacsar1998dynamic}, where no agent has an incentive to deviate from its current policy. This concept is applicable in both cooperative and competitive environments, with many MARL algorithms designed to converge to this point \cite{zhang2021decentralized}.

% \begin{definition}
% \textbf{(Nash equilibrium of the MG)}
% $\left( \mathcal{N}, \mathcal{S}, \{A^{i}\}_{i \in \mathcal{N}}, \mathcal{P}, \{R^{i}\}_{i \in \mathcal{N}}, \gamma \right)$ is a joint policy $\pi^* = 
% \left(\pi^{1,*}, \pi^{2,*}, \ldots, \pi^{N,*}\right)$, such that for any $s \in \mathcal{S}$ and $i \in \mathcal{N}$, there is 
% $V^{i}_{\pi^{i,*},\pi^{-i,*}}(s) \geq V^{i}_{\pi^{i},\pi^{-i,*}}(s)$, for any $\pi^{i}$.
% \end{definition}

% \subsubsection{Fully Cooperative}

% In a fully cooperative setting, all agents work together towards a common objective. Homogeneous agents typically perform more effectively under a shared reward function, while heterogeneous agents benefit from a reward sum system that accounts for their diverse capabilities and roles.

% \begin{itemize}
%     \item \textit{Reward Sum:}  \(\bar{R}(s,a,s') = N^{-1} \cdot \sum_{i \in N} R^{i}(s,a,s')\)\\ 
%     By focusing on the average reward, this approach encourages diverse agents to contribute according to their unique strengths whilst ensuring the team's overall performance is prioritized.

%     \item \textit{Shared Reward:} \( R_1 = R_2 = \dots = R_N = R \)\\ 
%     A special case of the reward sum, where all agents receive the same reward, ensuring uniform motivation to achieve the group's objectives, naturally motivating agents to work together and support each other's actions.
% \end{itemize}

% \subsubsection{Fully Competitive}

% In a fully competitive setting, agents compete against each other, often within a zero-sum framework where one agent's gain is equivalent to another's loss. This scenario is typical in duel-agent setups or games where only one winner can emerge \cite{silver2016mastering}.

% \begin{itemize}
%     \item \textit{Zero-Sum Game:} For two agents, \( R_1 + R_2 = 0 \). \\ The reward for one agent is the exact negative of the other’s reward \cite{littman1994markov}, reinforcing direct competition.
% \end{itemize}


% \subsubsection{Mixed}

% In a mixed setting, multi-agent systems have no constraints on the interactions and objectives of agents \cite{du2023review}. Examples include agents acting entirely based on individual interests within a \textit{general-sum game} framework \cite{hu2003nash}, or scenarios with two teams engaged in \textit{zero-sum competition} \cite{jaderberg2019human}, involving both fully cooperative and fully competitive agents.

% \subsection{Communication in a Multi-Agent System}

% Effective communication in a multi-agent system involves deciding what information to share, with whom, and when. Zhang et al. \cite{zhang2021multi} categorize communication structures in multi-agent systems into three types: centralized, where agents share local observations with a global controller that directs their actions; decentralized with networked agents, where agents share information directly with each other in a peer-to-peer network; and fully decentralized, where agents operate based solely on local information without direct communication with other agents.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/marl-information-structures.png}
%     \caption{Categories of communication structures in Multi-Agent Systems \cite{zhang2021multi}.}
%     \label{fig:marl-information-structures}
% \end{figure}

% \section[Multi-Agent RL]{Multi-Agent Reinforcement Learning}

% The complexities of multi-agent systems necessitate advanced learning algorithms for managing interactions and coordination among agents.  Multi-Agent Reinforcement Learning (MARL) builds on reinforcement learning principles to address these challenges in environments with multiple agents. MARL introduces distinct challenges and opportunities, demanding novel approaches for effective learning and robust performance across a wide range of multi-agent applications.

% \vspace{12pt}

% Given the rapid growth of research on MARL and the extensive body of literature available, this section will focus on methods specifically suited for large-scale network packet routing. This problem can be best described as a fully cooperative, distributed control challenge involving decentralized agents, with the simplifying assumptions of a single shared objective and homogeneous agents. The review will highlight the most effective techniques for addressing these challenges.

% \subsection{Decentralized Learning}

% The most straightforward approach is to consider each agent as an independent single-agent reinforcement learning problem. This approach assumes agents make decisions based solely on their local observations without any coordination or data aggregation \cite{zhang2021multi}. Consequently, decentralized learning approaches are infinitely scalable and maximally private, finding broad applications in fields such as autonomous driving \cite{zhang2023high}.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/auto-driving.jpg}
%     \caption{Application of cooperative decentralized learning within autonomous driving. In scenarios such as lane merging, agents must learn cooperative behavior without direct communication, relying on local observations to make decisions. \cite{malik2021collaborative}}
%     \label{fig:autonomous-driving}
% \end{figure}

% \subsubsection{Decentralised Partially Observable Markov Decision Process}

% With decentralized learning, multiple agents execute solely based on local observations. To formalize this, we extend the single-agent POMDP to the \textit{Decentralised POMDP (Dec-POMDP)} defined by the tuple $(S, \{A_i\}, P, R, \{\Omega_i\}, O, \gamma)$:

% \begin{itemize}
%     \item $S$: The set of states in the environment.
%     \item $A_i$: The set of actions for agent $i$, where $A = \prod_i A_i$ is the set of joint actions.
%     \item $P$: The state transition model, $T(s, a, s') = P(s' | s, a)$.
%     \item $R: S \times A \rightarrow \mathbb{R}$: The reward function.
%     \item $\Omega_i$: The set of observations for agent $i$, where $\Omega = \prod_i \Omega_i$ is the set of joint observations.
%     \item $O$: The observation probability function $O(s', a, o) = P(o|s', a)$.
%     \item $\gamma \in [0, 1]$: The discount factor.
% \end{itemize}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.65\linewidth]{figures/dec-POMPD.png}
%     \caption{Dec-POMPD: At time-step $t$, the environment is in state $s_t$ and emits a joint observation $o_t$. Each agent $i$ receives observation $o_{i,t}$, takes action $a_{i,t}$, forming joint action $\vec{a}_t$. The environment transitions to state $s_{t+1}$ and emits reward $r_t$. \cite{willemsen2021mambpo}}
%     \label{fig:Dec-POMPD}
% \end{figure}


% \subsubsection{Decentralized Value-Based Learning}
% \label{sec:independent-value-shared}

% In fully cooperative settings with homogeneous agents, the value function is consistent across all agents. This uniformity allows them to operate as a single decision-making entity by sharing parameters, which facilitates the application of single-agent RL techniques like Q-learning \cite{watkins1989learning}.

% \addvspace{12pt}

% Tan introduced the concept of \textit{Independent Q-Learning (IQL)} \cite{tan1993multi}, where agents independently learn policies based on their local observations to maximize a shared reward. In this framework, the transition probability for an agent \(i\) depends on the current state \(s\), its action \(a_i\), and the joint policies of the other agents \(\pi_{-i}\):

% \begin{equation}
% P_i(s'|s, a_i) = \sum_{a_{-i}} P(s' | s, a_i, a_{-i}) \pi_{-i}(a_{-i} | s)
% \end{equation}

% \begin{equation}
% \label{eq: IQL}
% Q_i(s, a_i) = \mathbb{E}_{P_i(s' | s, a_i)} \left[ r + \gamma \max_{a'_i} Q_i(s', a'_i) \right]
% \end{equation}

% As agents update their policies using IQL, the non-stationarity of the transition probabilities \(P_i\) hinders guaranteed convergence to a Nash equilibrium. However, \textit{MA2QL} \cite{su2022ma2ql} addresses this by allowing agents to alternate their learning updates, ensuring stationary transition probabilities and convergence when trained on-policy.

% \vspace{12pt}

% Most practical Q-learning implementations rely on the DQN \cite{mnih2013playing}. However, as Q-learning is an off-policy algorithm, the relevance of experiences generated with non-stationary policies and transition probabilities, often compromises the replay mechanism. To address this, Foerster et al. \cite{foerster2016ddrqn} initially removed the replay buffer, and later introduced two selective sampling strategies: Importance Sampling, which decays outdated data to prioritize recent experiences, and Fingerprinting, a Meta Reinforcement Learning approach that stores iteration numbers and exploration rates within the state to assess the relevance of past experiences \cite{foerster2017stabilising}.

% \vspace{12pt}

% Without access to joint actions, each agent estimates its Q-value based on individual actions, making value estimations vulnerable to the negative exploration of other agents in a shared reward setting. To mitigate this, \textit{Distributed Q-learning} \cite{lauer2000algorithm} updates the value function only with a guaranteed improvement (positive TD error), though it's limited to deterministic environments. \textit{Hysteretic Q-learning} \cite{matignon2007hysteretic} extends this approach to stochastic environments by applying a higher learning rate when the TD error is positive.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\linewidth]{figures/drqn-architecture.png}
% \caption{DRQN architecture with a convolutional encoder feeding into an LSTM network, which uses past observations to generate Q-values.  \textcolor{blue}{Source for this??? }}
% \label{fig}
% \end{figure}

% Another approach to addressing non-stationarity involves enabling agents to store and utilize past experiences. The \textit{Deep Recurrent Q-Network (DRQN)} \cite{hausknecht2015deep} replaces the first post-convolutional feed forward layer in a DQN with an LSTM, allowing the agent to retain memory of past observations. The \textit{Deep Distributed Recurrent Q-Network (DDRQN)} \cite{foerster2016ddrqn} builds on this by conditioning policy decisions on the previous action, using recurrent memory to approximate the agent's policy history.

% \subsubsection{Decentralized Policy-Based Learning}
% \label{sec:independent-policy-shared}

% In highly non-stationary environments, policy-based methods have a significant advantage due to their direct parameterization of the policy. This approach theoretically makes them better suited to adapt dynamically to the changing policies of other agents. However, in practice, the first decentralized policy-based method, \textit{Independent Actor-Critic (IAC)} \cite{foerster2018counterfactual}, demonstrated relatively suboptimal performance, as this advantage was outweighed by the instability caused by large policy updates from other agents.

% \vspace{12pt}

% De Witt et al. introduced \textit{Independent Proximal Policy Optimization (IPPO)} \cite{de2020independent}, a decentralized multi-agent variant of \textit{PPO} \cite{schulman2017proximal}. IPPO employs policy update clipping, defined by the loss function in Equation \ref{eq:ippo-loss}, which enhances the stability of transition probabilities. This approach allows agents to adapt more effectively to evolving policies, outperforming decentralized value-based learning methods and achieving performance levels comparable to centralized training with decentralized execution (CTDE) methods in certain environments.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/trpo.png}
%     \caption{Illustration of the unconstrained optimization process using the trust-region method. As optimization progresses, the trust region progressively shrinks, enhancing convergence stability \cite{wenhe2014trust}.}
%     \label{fig:trust-region-method}
% \end{figure}

% Building on the success of IPPO, recent research has focused on policy clipping. \textit{Decentralized Policy Optimization (DPO)} \cite{su2022decentralized} extends the single-agent \textit{Trust Region Policy Optimization (TRPO)} \cite{schulman2015trust} to multi-agent settings. TRPO constrains policy updates within a "trust region," limiting the Kullback-Leibler (KL) divergence \cite{kullback1951information} between new and old policies. The state-of-the-art in decentralized learning, \textit{Total Variation Policy Optimization (TVPO)} \cite{su2024general}, introduces \( f \)-divergence for measuring distributional distance, with KL divergence as a special case. The optimization details of TVPO are beyond the scope of this report.

% \subsection{Centralized Learning}
% \label{sec:centralised-learning}

% A common yet naive approach to solving multi-agent problems is to treat them as a single-agent problem by using a centralized controller to determine the entire joint action \( a = (a_1, a_2, \ldots, a_N) \). While this method, known as \textit{Centralized Training with Centralized Execution (CTCE)}, may work for smaller systems, it becomes impractical for large-scale problems due to the exponentially growing action space as the number of agents increases. This results in significant computational challenges during training and can render the approach intractable during execution in larger systems.

% \subsubsection{Centralised Training Decentralised Execution}

% The \textit{Centralized Training with Decentralized Execution (CTDE)} framework is designed to optimize agent policies using substantial computational resources in an offline setting. During training, a central controller gathers and processes information from all agents to optimize their collective policies. Once training is complete, each agent operates independently, executing the learned policies without further centralized coordination. This approach leverages the strengths of centralized learning while maintaining the flexibility and scalability of decentralized execution. Key advantages and disadvantages of this framework are summarized in Table \ref{table:ctde_pros_cons}. 

% \begin{table}[H]
% \centering
% \caption{Advantages and Disadvantages of CTDE in Multi-Agent Systems}
% \label{table:ctde_pros_cons}
% \begin{tabular}{ p{0.47\textwidth}|p{0.47\textwidth} }
% \hline
% \textbf{Advantages} & \textbf{Disadvantages} \\
% \hline
% \textbf{Improved Observability:} The central controller uses aggregated observations to better estimate the environment's true state & \textbf{Scalability Issues:} Combinatorial nature of MARL makes centralized training computationally expensive / impractical for large-scale systems. \\
% \hline
% \textbf{More Stationarity:} Coordinated policy updates reduce the need for agents to adapt to independently evolving policies. & \textbf{Communication Overhead:} Fast and effective communication channels are required during training, which can be difficult to maintain over large scales. \\
% \hline
% \textbf{Effective Credit Assignment:} A global view allows the central controller to better assign rewards based on the collective performance of agents. & \textbf{Privacy Concerns:} The requirement to aggregate information from all agents can lead to privacy issues in sensitive environments. \\
% \hline
% & \textbf{Robustness:} The central controller can become a bottleneck or a single point of failure. \\
% \hline
% & \textbf{Availability:} In certain systems, a central controller may not be feasible or available. \\
% \hline
% \end{tabular}
% \end{table}


% \subsubsection{Factorising the Joint Action Space}

% To retain the benefits of centralized training while enabling decentralized execution, CTDE algorithms must learn to factorize the joint action space. Qu et al.\ \cite{qu2020intention} categorize these approaches into two main groups:

% \begin{itemize}
%     \item \textbf{Policy Factorization:} $\pi(a|s) := \prod_{i=1}^N \pi_i(a_i|s)$ \\
%     This approach assumes that policies are independent, generally requiring a centralized critic network to coordinate behavior for stable learning.

%     \item \textbf{Value Function Factorization:} $Q_{\text{tot}}(s, a) = f (Q_1(s, a_1), Q_2(s, a_2), \dots, Q_N(s, a_N))$ \\
%     This method factorizes the joint value function into separate independent evaluations, each focused on the actions of a single agent, with \( f \) representing the factorization function.
% \end{itemize}

% \subsubsection{Policy Factorization}

% In policy factorization, a central critic network oversees training by aggregating local observations from each actor network to generate a central value estimate. This estimate guides the updates to the actor networks' policies. In the shared reward setting, a single centralized critic network is sufficient. However, in the reward sum setting, each agent requires its own fully observable critic network.

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.5\linewidth]{figures/fully-observable-critic.png}
% \caption{Fully observable critic in the Reward Sum setting: Agents share their observations and actions with all critic networks. The total value across these networks is used to shape the agents' policies \cite{oroojlooy2023review}.}
% \end{figure}

% Single-agent actor-critic algorithms, such as \textit{Deep Deterministic Policy Gradient (DDPG)} \cite{lillicrap2015continuous}, have been extended to multi-agent settings, resulting in \textit{Multi-Agent Deep Deterministic Policy Gradient (MADDPG)} \cite{lowe2017multi}.  MADDPG maintains the fundamental structure of DDPG, sampling trajectories from a shared replay buffer and employing separate target networks. However, in the multi-agent setting, each agent learns its policy while considering the actions of other agents. The deterministic policy gradient update is modified to account for the joint action space, as shown in the following equation:

% \begin{align}
%     \nabla_{\theta_i}J(\mu_i) = \mathbb{E}_{a_{-i}, s}[\nabla_{\theta_i}\mu_i(a_i|s_i)\nabla_{a_i}Q^{\mu^{\prime}_i}(s, a_1, \ldots, a_N)].
%     \label{eq:MADDPG}
% \end{align}

% Another prominent algorithm is \textit{Multi-Agent Proximal Policy Optimization (MAPPO)} \cite{yu2022surprising}, an adaptation of PPO \cite{schulman2017proximal} within the CTDE framework. MAPPO challenges the traditional belief that on-policy methods, like PPO, are less sample efficient in multi-agent scenarios.  By enabling parameter sharing among agents, MAPPO improves sample efficiency, particularly in homogeneous or cooperative environments.

% \vspace{12pt}

% Even with a central controller, credit assignment remains challenging in shared reward settings. Foerster et al. introduced \textit{Counterfactual Multi-Agent Policy Gradient (COMA)} \cite{foerster2018counterfactual} to address this. COMA improves credit assignment by using a counterfactual baseline instead of the value function \( V(s_t) \) for advantage estimation. To isolate the effect of each agents actions, it calculates a counterfactual value for each agent, reflecting the expected return if the agent had taken the average action \( a'_i \) rather than its actual action \( a_i \), while keeping other agents' actions \( a_{-i} \) fixed. The counterfactual baseline \( b(s, a_{-i}) \) and counterfactual advantage \( A(s, a_i, a_{-i}) \) are defined below. 

% \begin{equation}
% b(s, a_{-i}) = \sum_{a'_i} \pi_i(a'_i|s) Q(s, a'_i, a_{-i})
% \label{eq:counterfactual-baseline}
% \end{equation}
% \begin{equation}
% A(s, a_i, a_{-i}) = Q(s, a_i, a_{-i}) - b(s, a_{-i})
% \label{eq:counterfactual-advantage}
% \end{equation}

% Centralized approaches often struggle to aggregate information from all agents in large multi-agent systems. The \textit{Multi-Actor-Attention-Critic (MAAC)} algorithm \cite{iqbal2019actor} addresses this challenge by building on the \textit{Soft Actor-Critic (SAC)} single agent algorithm \cite{haarnoja2018soft}. SAC is known for its sample efficiency and faster convergence, achieved by maximizing both the expected reward and policy entropy, thereby encouraging exploration.  MAAC uses a shared attention mechanism \cite{bahdanau2014neural} to efficiently integrate observations for the central critic, allowing it to focus on the most relevant information from each agent.

% \subsubsection{Value Function Factorization}

% To factorize the joint policy, the central critic must coordinate behavior across all agents, which requires considering the entire joint-action space. A more efficient approach is to use localized critic networks and factorize only the value function. In this setup, agents share their local value estimates \( Q_i \) with a central controller, which serves as a mixing network to produce a global value estimate \( Q_{\text{tot}} \). These individual value functions are then tailored to guide the policies of decentralized actor networks during execution.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/value-factorisation.png}
%     \caption{Value Factorization The joint action-value function \(Q_{\text{tot}}\) is decomposed into individual value functions \(Q_0, \dots, Q_N\), allowing each agent to select actions by maximizing their respective \(Q_i\) based on local observations \(\mathbf{o}^t_i\) during execution \cite{oroojlooy2023review}.}
%     \label{fig:value-factorisation}
% \end{figure}

% The mixing network must maintain the factorization of the joint-action value function and satisfy the \textit{Individual-Global Maximization (IGM)} constraint \cite{rashid2020monotonic} as defined in Equation \ref{eq:IGM}. Factorization allows the global value to be decomposed into individual components, while the IGM constraint ensures that maximizing the global action-value function corresponds to independently maximizing each agent’s individual action-value function. Here, \( \tau \) represents the vector of local observation-action histories, and \( a \) is the joint-action vector.

% \begin{align}
%     \text{argmax}_{a} Q_{\text{tot}}(\tau, a) = \left( \text{argmax}_{a_1} Q_1(\tau_1, a_1), \ldots, \text{argmax}_{a_n} Q_n(\tau_n, a_n) \right)
% \label{eq:IGM}
% \end{align}

% Value factorization methods differ in how they factorize the global value function. The simplest and earliest approach is the \textit{Value Decomposition Network (VDN)} \cite{sunehag2017value}, where the mixing network produces the joint-action value function, \( Q_{\text{tot}} \), as a summation of the action values from decentralized critics, \( Q_i \). This method satisfies the IGM constraint and is highly scalable; however, linear factorization has limited representational capacity and offers no global convergence guarantee \cite{du2023review}.

% \begin{align}
%     Q_{\text{tot}}(\tau, a) = \sum_{i} Q_i(\tau_i, a_i)
% \label{eq:VDN}
% \end{align}

% To better represent complex agent interactions, Rashid et al. proposed \textit{QMIX} \cite{rashid2020monotonic}, which relaxes the strict summation factorization condition. Instead, it requires that the joint-action value function \( Q_{\text{tot}} \) be monotonically increasing with respect to each action value \( Q_i \). This approach still satisfies the IGM constraint and allows the summation to be replaced by a neural network mixing network, provided all weights are non-negative.

% \begin{align}
%     \frac{\partial Q_{\text{tot}}}{\partial Q_i} \geq 0, \forall i.
% \label{eq:QMIX}
% \end{align}

% Several variations have been developed to create more flexible mixing networks. \textit{QTRAN} \cite{son2019qtran} relaxes the monotonicity constraint by transforming the joint-action value function into an alternative that closely tracks the original but can be additively decomposed into individual components. \textit{QPLEX} \cite{wang2020qplex} reformulates the IGM constraint as an advantage-based IGM by separating \( Q_i(o_i, a_i) \) into a value function \( V(s) \) and an advantage function \( A_i(o_i, a_i) \).

% \vspace{12pt}

% Value factorization methods are susceptible to \textit{relative overgeneralisation} \cite{wei2016lenient}, where monotonic factorization fails to capture non-monotonic team reward functions, leading to suboptimal joint policies \cite{de2020independent}. To represent non-monotonic interactions, some methods frame interactions using a \textit{Coordination Graph (CG)} approach. Derived from graphical game theory, this approach factorizes each agent's value into a \textit{utility} function, representing the individual’s contribution to the overall outcome, and a \textit{payoff} function, accounting for the pairwise impact of actions on other agents.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/value-factorisation-graphs.png}
%     \caption{Graphical Value Factorization \cite{bohmer2020deep}: (a) VDN \cite{sunehag2017value} sums independent utility functions, corresponding to an unconnected coordination graph; (b) QMIX \cite{rashid2020monotonic} uses a monotonic mixture of utilities, representable as a sum of pairwise payoffs; (c) QTRAN \cite{son2019qtran} assumes no factorization and is represented as a single hypergraph connecting all nodes.}
% \label{fig:graphical-value-factorisation}
% \end{figure}

% Building on this principle, \textit{Deep Coordination Graphs (DCG)} \cite{bohmer2020deep} decompose the value function using two neural networks for each agent: one estimates individual utility, while the other estimates the shared payoff function. This approach captures complex agent interactions and mitigates relative overgeneralization. A more general method involves learning agent-agent interactions with a \textit{Graph Neural Network (GNN)} \cite{scarselli2008graph}, specifically designed for graph-structured data. Instead of using two separate networks, \textit{GraphMix} \cite{naderializadeh2020graph} employs a single mixing GNN to derive a global value function from individual agent value functions.

% \subsection{Decentralised Learning with Networked Agents}

% Dec-POMPD provides a powerful framework for multi-agent systems but is provably intractable to solve \cite{oliehoek2013approximate, tan1993multi}, with a computational complexity class of NEXP-complete \cite{amato2013decentralized}. Consequently, research has focused on restricted variations of the Dec-POMPD that are easier to solve yet represent many practical applications. 

% \vspace{12pt}

% A special case of the Dec-POMPD considers agents exchanging or sharing local information across a time-varying communication network. When communication is free, instantaneous, and lossless, the system effectively becomes centralized and therefore solvable as a POMPD \cite{oliehoek2012tree}, as all agents have access to all observations at each step. However, in practical applications, the challenge lies in creating a communication network that minimizes delay, cost, and information loss, thereby approximating centralized performance while maintaining the scalability, robustness, and privacy benefits of a decentralized system. There are three primary categories of approaches:

% \begin{table}[H]
% \centering
% \caption{Categories of Approaches for Networked MARL in Decentralized Systems}
% \label{tab:marl-methods}
% \begin{tabularx}{\textwidth}{>{\raggedright}p{3cm}>{\raggedright\arraybackslash}X}
% \hline
% \textbf{Category} & \textbf{Description} \\ \hline

% Mean Field & Uses Mean-field Theory \cite{stanley1971phase}  to approximate interactions between a single agent and the averaged effect of the entire population, simplifying multi-agent dynamics. \\ \hline 

% Consensus Mechanism & Agents iteratively share information with neighbors to reach agreement on certain variables, enabling coordinated actions. \\ \hline

% Communication Protocol & Defines or learns strategies for information sharing among agents, including rules for with whom, when, what, and how to communicate. \\ \hline
     
% \end{tabularx}
% \end{table}

% \subsubsection{Network Topology}

% The topology of a communication network is crucial in decentralized systems, as it defines how agents are connected and interact. Key topologies include \textit{Peer-to-Peer}, where agents communicate directly and equally, and \textit{Hierarchical}, where communication flows through structured levels of importance. Topologies can be \textit{static}, with fixed connections determined by factors such as proximity, or \textit{dynamic}, evolving over time through adaptive mechanisms or changing external conditions. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/network-topology.png}
%     \caption{Network Topologies: Peer-to-Peer (blue), Hierarchical (green), Dense (red), and Sparse (yellow)}
%     \label{fig:network-topology}
% \end{figure}

% Additionally, networks can be \textit{dense}, with each agent interconnected and connections scaling quadratically with agents, or \textit{sparse} with only a subset of agents directly connected. These topological structures determine the network's efficiency, scalability, and resilience.

% \subsubsection{Mean Field Theory}

% Originating from physics, Mean Field Theory (MFT) \cite{stanley1971phase} simplifies complex many-agent interactions by approximating them as two-agent interactions, reducing the problem to a fixed point equation in cooperative Mean Field Control (MFC). This approach allows the approximation of a finite N-agent system using mean-field methods, facilitating the application of learning algorithms without the need to directly solve the finite system. In large systems, the MFC solution is nearly optimal, converging to a Pareto Optimum \cite{cui2022survey}.

% \begin{definition}
% \textbf{(Pareto Optimum)} A policy is a Pareto efficient solution if it is not dominated by any other policy, meaning no agent's policy can be improved without harming another agent's policy.
% \end{definition}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.4\linewidth]{figures/mean-field-theory.png}
% \caption{Mean field approximation: each agent (node) is influenced by the mean effect of its neighbors (blue area) \cite{yang2018mean}.}
% \label{fig:mean-field-approx}
% \end{figure}

% Yang et al. \cite{yang2018mean} pioneered the use of MFT in MARL with two algorithms: MF-Q (Q-learning) and MF-AC (actor-critic).  These algorithms decompose the $Q$-function by focusing on the value of pairwise local interactions, denoted as $Q^i(s, a^i, a^j)$, where agent $i$ interacts with its neighboring agents $j$. Using a mean-field approximation, these pairwise interactions are reduced into interactions between each agent $i$ and a virtual "mean agent," represented by $Q^i(s, a^i, \bar{a}^i)$. The virtual mean agent relies on the average action $\bar{a}^i$, calculated from the actions $a^j$ of agent $i$'s neighbors.

% \vspace{12pt}

% However, MF-Q and MF-AC assume symmetric, unweighted interactions among homogeneous agents, which limits their representational capacity. To address this, the \textit{Graph Attention Mean Field (GAT-MF)} method proposed by Hao et al. \cite{hao2023gat} introduces a graph attention mechanism to dynamically adjust the strength of interactions, achieving superior performance compared to state-of-the-art methods in multi-agent systems with over 3,000 agents. Despite these advancements, MFT-based approaches fundamentally rely on the assumption that the influence of other agents can be approximated by an average effect. This assumption restricts their effectiveness to environments with homogeneous agents and similar policies, resulting in poor approximation accuracy and suboptimal performance in more complex, heterogeneous environments with diverse agent behaviors and interactions.

% \subsubsection{Consensus Mechanism}

% Constraining information transfer to a subset of local nodes is a common technique in distributed optimization for static or one-stage decision-making problems \cite{xiao2007distributed}. This approach leverages the locality of interaction, assuming weak coupling between policies and observations of distant agents, which is reasonable for large-scale multi-agent systems \cite{nair2005networked}. However, applying this method to sequential decision-making, where decisions have long-term impacts, presents significant challenges.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\linewidth]{figures/consensus.png}
%     \caption{Consensus Network \cite{oroojlooy2023review}: A network where each node \( i \) exchanges information with its immediate neighbors to achieve consensus on a shared variable.}
%     \label{fig:consensus-network}
% \end{figure}

% Consensus approaches can be divided into \textit{policy learning} and \textit{policy evaluation}. Policy learning focuses on developing an optimal control policy for all agents, while policy evaluation aims to learn the optimal value function for a fixed, possibly suboptimal, multi-agent policy \cite{li2023f2a2}.

% \vspace{12pt}

% \textit{Policy Learning}

% \vspace{12pt}

% Most policy learning approaches are centred on the two algorithms proposed by Zhang et al. \cite{zhang2018fully}. Each agent \( i \) maintains its own parameter \( \omega^i \) and uses \( Q(\cdot, \cdot; \omega^i) \) as a local estimate of \( Q_\theta \). The agents update their parameters using the TD error, followed by a weighted combination step with neighbor estimates \(\tilde{\omega}^j_t\) using the network edge weights \( c_t(i, j) \), as described in the equation below.

% \begin{align}
% \label{eq: zhang_alg1_c4}
%     \omega^i_{t+1} = \sum_{j \in \mathcal{N}} c_t(i, j)  \cdot \tilde{\omega}_t^j
% \end{align}

% This approach can be seen as a distributed variant of COMA \cite{foerster2018counterfactual}, where each agent estimates \( Q(\cdot, \cdot; \omega^i) \) for the counterfactual baseline \( Q_\theta \) and uses a consensus constraint to minimize differences. Zhang et al. were the first to provide provable convergence guarantees under this reward setting. However, this comes at the cost of requiring full observability of the global state and joint actions, making it unsuitable for large-scale distributed control problems. Additionally, the parameter-sharing mechanism allows network-wide collaboration while preserving privacy by not revealing individual rewards or policies \cite{zhang2021decentralized}.

% \vspace{12pt}

% \textit{Policy Evaluation}

% \vspace{12pt}

% In policy evaluation, agents aim to minimize the Mean Square Projected Bellman Error (MSPBE) to learn the optimal value function for a fixed joint policy. While the Bellman equation (Equation \ref{eq: bellman}) recursively computes the value function, exact computation is impractical with function approximators. Therefore, the true value function is projected onto a smaller space defined by the approximator, resulting in the Projected Bellman Error, which measures the error in this projection. In multi-agent settings, MSPBE quantifies the average squared Mahalanobis distance between each agent's projected value function and its Bellman update.

% \vspace{12pt}

% Minimizing MSPBE is a standard objective in multi-agent policy evaluation methods \cite{macua2014distributed, stankovi2016multi, wai2018multi}. However, most work focuses on proving convergence rather than developing practical algorithms. These methods assume a fixed policy, making it impractical to compute MSPBE after each policy update in dynamic systems. Additionally, evaluating the joint policy to compute MSPBE becomes infeasible in large multi-agent systems.

% \subsection{Communication Protocols}
% \label{sec:communication-protocols}

% Fundamentally, Mean Field and Consensus Mechanism approaches are restricted special cases of communication protocols. Applications like Network Packet Routing, which involve distributed agents with partial observability and heterogeneous policies, demand more general and robust communication protocols.

% \vspace{12pt}

% Effective communication relies on a shared language and understanding of symbols between speaker and listener \cite{skyrms2010signals}. This can be established through predefined protocols or learned by agents, with recent work favoring the latter for greater flexibility and adaptability \cite{wagner2003progress}. Communication can be either \textit{discrete}, using a finite set of symbols, or \textit{continuous}, with values that vary within a range.

% \vspace{12pt}

% Agents usually transmit messages via a shared communication channel \cite{foerster2016learning}, though they can also communicate directly through actions \cite{grupen2020low}. Messages may be exchanged before actions \cite{sukhbaatar2016learning}, concurrently \cite{foerster2016learning}, or across multiple rounds before making a decision \cite{weil2024towards}.

% \vspace{12pt}

% Learnable communication protocols are defined by four key factors: message content (what is communicated), message recipients (who receives the information), message aggregation (how the information influences decision-making), and the learning mechanism (how the protocol is developed).

% \subsubsection{Message Content}

% Encoding local observations often involves using a learnable neural network, such as a Feed-Forward Network, RNN, CNN, or GNN. For effective communication, it's crucial that all agents share a mutual understanding of these observations to ensure message consistency and interpretability. In centralized training, this is straightforward as parameters can be shared among agents. However, in decentralized training, the challenge is greater, as protocols map action-observation histories to sequences of messages, leading to a high-dimensional protocol space \cite{foerster2016learning}. While there is extensive research on maintaining consistent encodings across decentralized agents \cite{lin2021learning, lo2023learning, yuan2021graphcomm, muller2024clustercomm}, this falls outside the scope of this report.


% \subsubsection{Message Recipients}

% The next step is to determine which agents should receive the transmitted information. Early approaches, like \textit{CommNet} \cite{sukhbaatar2016learning}, broadcast observations to all agents, forming a dense static network. However, this approach causes communication overhead to scale quadratically with the number of agents, leading to a computationally burdensome network and overwhelming agents with potentially irrelevant information. To avoid overwhelming agents, \textit{NeurComm} \cite{chu2020multi} broadcasts messages but applies a spatial discount factor to weight incoming communications. Externally constrained approaches such as the \textit{DGN} \cite{jiang2018graph} select recipients based on factors such as proximity and cost. However in dynamic systems, time-varying external factors can easily disrupt collaboration and learning. 

% \vspace{12pt}

% \textit{Targeting Mechanisms}

% \vspace{12pt}

% Targeting mechanisms form sparse networks, mitigating irrelevant information overload and maximizing efficiency by identifying the most relevant message recipients. Effectively selecting which agents should communicate generally requires a central overview with all current targeting mechanisms limited to the CTDE framework. 

% \vspace{12pt}

% Conventionally, targeting mechanisms use a key-query matching system. In \textit{TarMAC} \cite{das2019tarmac}, a learnable key is broadcasted with each message, encoding the intended recipient's properties. Recipients apply a soft-attention mechanism to assess message relevance, reducing information overload. The central controller shapes the key, determining which agents should interact. \textit{ATOC} \cite{jiang2018learning} reduces TarMAC's communication overhead by broadcasting only to agents within its observable range. It forms dynamic communication groups using a hard-attention mechanism with learnable keys and then restricts broadcasts to these groups for a set duration. 

% \vspace{12pt}

% \textit{When2Comm} \cite{liu2020when2com} builds on this key-query matching system, introducing \textit{asynchronous} communication. \textit{Synchronous} communication is inefficient due to the need for agents to wait for each other's messages. \textit{When2Comm} uses self-attention between the agent's own key and query vectors, assuming they will align closely when the agent has sufficient information to make a decision, signaling the end of communication.


% \begin{figure}[H]
% \centering
% \includegraphics[width=0.9\linewidth]{figures/when2comm_adj.png}
% \caption{When2Comm Adjacency Matrix: Rows with a self-attention score of 1 are replaced with an identity row, indicating no further communication is needed. Other rows are derived from scaled, pruned, and activated matching scores.}
% \label{fig}
% \end{figure}

% \textit{I2C} \cite{ding2020learning} takes a different approach, instead using a feed-forward network to map local observations to a belief about which individual agents to communicate with, eliminating broadcasting altogether. Using a similar idea, \textit{Model-Based Communication (MBC)} \cite{han2023model} trains agents to predict the content of incoming messages using supervised learning based on past communications. If an agent's confidence in its prediction falls below a certain threshold, it initiates a broadcast, ensuring messages are sent only when necessary.

% \vspace{12pt}

% For scalability, \textit{ATOC} and \textit{I2C} restrict communication to agents within the sender's observable range, which can lead to suboptimal convergence if distant agents are relevant. \textit{G2ANet} \cite{liu2020multi} addresses this by starting with a dense network and pruning irrelevant connections using a hard-attention gating mechanism. In contrast, \textit{AC2C} \cite{wang2023ac2c} takes the reverse approach, starting with local 1-hop connections and training a controller to selectively expand the most relevant 2-hop connections. Taking a completely different approach, \textit{MAGIC} \cite{niu2021magic} uses a graph attention encoder to directly learn adaptive, directed graphs that specify optimal communication links.

% \subsubsection{Message Aggregation}

% In the discussed methods, agents receive multiple messages, making it challenging to extract the most relevant information for policy decisions. For a communication protocol to be stable and effective, the output must remain consistent regardless of message order. Basic approaches include concatenating \cite{foerster2016learning, kim2019learning, kim2020communication}, averaging \cite{sukhbaatar2016learning, singh2018learning}, or summing \cite{du2021learning} the incoming message feature vectors. However, these methods struggle with scalability and can lead to information loss with large message volumes. To better identify critical information, some methods use handcrafted rules to unequally weight messages \cite{kim2019message}. Alternatively, order-invariant learnable mechanisms like soft-attention \cite{das2019tarmac} and bi-directional RNNs \cite{peng2017multiagent} dynamically determine message importance and process messages in both forward and backward directions.

% \vspace{12pt}

% \textit{Graph Convolutions}

% \vspace{12pt}

% For sparse graphs, Graph Convolutional Networks (GCNs) \cite{kipf2016semi} aggregate information by leveraging graph structure. GCNs encode node or edge features into low-dimensional representations, iteratively updating them by aggregating information from neighboring nodes or edges, typically using a weighted sum or average. This process captures both individual node features and overall graph structure. GCNs use the adjacency matrix to define node connectivity and guide aggregation. To stabilize training, the adjacency matrix is often normalized, balancing the influence of neighboring nodes. Algorithm \ref{alg:gcn} outlines a basic graph convolutional layer:

% \addvspace{12pt}

% \begin{algorithm}[H]
% \caption{Graph Convolutional Layer}
% \label{alg:gcn}
% \KwIn{Adjacency matrix $A$, Input Feature matrix $X$, Graph Weight matrix $W$, Activation function $\sigma$}
% $D_{ii} \gets \sum_{j} A_{ij}$ \tcp*{Compute degree matrix}
% $\tilde{A} \gets D^{-\frac{1}{2}} A D^{-\frac{1}{2}}$ \tcp*{Normalize adjacency matrix}
% $H \gets \sigma(\tilde{A} X W)$ \tcp*{Apply transformation and activation}
% \textbf{return:} Updated feature matrix $H$\;
% \end{algorithm}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.78\linewidth]{figures/graph_and_adj_matrix.png}
%     \caption{Undirected graph (left) and corresponding adjacency matrix (right) which represents node connections numerically.}
%     \label{fig:graph_adj_matrix_gcn}
% \end{figure}

% The main limitation of GCNs is their static weighting of messages from neighboring nodes, which fails to capture the varying importance of information that may change dynamically over time. Graph Attention Networks (GATs) \cite{velivckovic2017graph} overcome this by using an attention mechanism to dynamically weight messages from neighbors, as illustrated in Figure \ref{fig:gat_diagram}. Algorithm \ref{alg:gat} presents a single GAT layer. 

% % \addvspace{12pt}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/gat.png}
%     \caption{GAT \cite{velivckovic2017graph}: Computing attention coefficients using a shared mechanism across node pairs (left). Using these coefficients to compute the weighted sum of neighboring node features, updating each node's feature representation (right).}
%     \label{fig:gat_diagram}
% \end{figure}

% \addvspace{12pt}

% \begin{algorithm}[H]
% \caption{Graph Attention Layer}
% \label{alg:gat}
% \KwIn{Adjacency matrix $A$, Input feature matrix $X$, Graph weight matrix $W$, Attention function $\alpha$, Activation function $\sigma$}
% $H' \gets XW$ \tcp*{Apply linear transformation}
% \ForEach{edge $(i, j) \in A$}{
%     $e_{ij} \gets \alpha(H'_i, H'_j)$ \tcp*{Compute attention score}
%     $\alpha_{ij} \gets \frac{\exp(e_{ij})}{\sum_{k \in \mathcal{N}(i)} \exp(e_{ik})}$ \tcp*{Normalize attention scores}
% }
% \ForEach{node $i \in A$}{
%     $H_i \gets \sigma\left(\sum_{j \in \mathcal\{N(i)\}} \alpha_{ij} H'_j\right)$ \tcp*{Apply weighted aggregation and activation}
% }
% \textbf{return} Updated feature matrix $H$\;
% \end{algorithm}

% \addvspace{12pt}

% Using graph convolutional layers within message-passing systems to aggregate messages is common. For instance, the \textit{Deep Implicit Coordination Graph (DICG)} \cite{li2020deep} and DGN \cite{jiang2018graph} utilize GCNs, while MAGIC \cite{niu2021magic} leverages GATs. A key advantage of these layers is their ability to be stacked, effectively enabling multi-round communication. This stacking increases the receptive field, allowing agents to propagate long-range information through multiple hops while only communicating with direct neighbors, thus expanding the receptive field efficiently without significant communication overhead

% \subsubsection{Learning Mechanism}

% The final aspect to consider for learnable communication-based protocols is how they utilize feedback to improve the protocol. Learnable protocols can be characterized as either \textit{Reinforced} or \textit{Differentiable}, as detailed in Table \ref{tab:learning_mechanisms}.

% \begin{table}[H]
% \centering
% \caption{Comparison of Learning Mechanisms for Communication Protocols}
% \label{tab:learning_mechanisms}
% \begin{tabular}{ p{3cm} p{8cm} p{3cm} }
% \hline
% \textbf{Mechanism} & \textbf{Description} & \textbf{Examples} \\ \hline
% Reinforced & Assumes successful communication leads to environmental rewards. Uses feedback from the environment to reinforce effective communication strategies, often with reinforcement learning. & \textit{RIAL} \cite{foerster2016learning}, \textit{ATOC} \hspace{0.7cm}\cite{jiang2018learning} \\ \hline
% Differentiable & Uses continuous feedback from other agents to refine communication through backpropagation, allowing real-time adjustments and improvement. Gradients are computed based on the difference in Q-values after receiving the message. & \textit{DIAL} \cite{foerster2016learning}, \textit{CommNet} \cite{sukhbaatar2016learning} \\ \hline
% \end{tabular}
% \end{table}

% \section{Network Packet Routing}

% Network packet routing is a fundamental aspect of computer networking that enables the transmission of data across different networks. This process involves directing data packets from a source node to a destination node through a series of intermediate nodes, such as routers and switches. The primary objectives of packet routing are to minimize \textit{latency} (the delay from source to destination) and ensure reliable data delivery by minimizing \textit{packet loss}.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/network-packet-routing.jpg}
%     \caption{Network packet routing from source to destination via intermediary routers, illustrating the selection of efficient paths based on routing protocols \cite{Kubilius2022network}.}
%     \label{fig:network-packet-routing}
% \end{figure}

% Routers, the primary devices responsible for packet routing, use routing tables to keep track of network paths and make forwarding decisions. When a packet arrives at a router, the router examines the packet's destination address and consults its routing table to decide the next hop. This process is repeated at each router along the path until the packet reaches its final destination.

% \subsection{Routing Protocols}

% Routing decisions rely on protocols that determine the optimal path based on network topology, traffic, and link cost. Common protocols include \textit{Routing Information Protocol (RIP)} \cite{hedrick1988routing}, \textit{Open Shortest Path First (OSPF)} \cite{sidhu1993open}, and \textit{Border Gateway Protocol (BGP)} \cite{rfc1105}. A comparison of these protocols is provided in Table \ref{tab:routing_protocols}.

% \begin{table}[H]
% \centering
% \caption{Comparison of RIP, OSPF, and BGP Routing Protocols}
% \begin{tabular}{p{2.2cm} p{2.2cm} p{9.8cm}}
% \hline
% \textbf{Protocol} & \textbf{Type} & \textbf{Description} \\ \hline
% RIP & Distance-vector & Uses hop count with a maximum of 15 hops. Regularly exchanges entire routing tables, leading to higher overhead and slower convergence. \\ \hline
% OSPF & Link-state & Uses Dijkstra's algorithm to compute the shortest paths. Maintains a map of the topology and exchanges link state advertisements (LSAs) for faster convergence, supporting larger, complex networks. \\ \hline
% BGP & Path-vector & Used for routing between autonomous systems (AS). Tracks the full AS path to the destination, preventing routing loops and enabling policy-based routing decisions, essential for reliable internet routing. \\ \hline
% \end{tabular}
% \label{tab:routing_protocols}
% \end{table}


% \subsection{MARL in Network Packet Routing}

% As networks grow in size and complexity due to the rise of data-intensive applications and the demand for more dynamic capabilities, traditional routing algorithms are becoming increasingly inadequate. A promising approach is the application of RL in network packet routing, which enables routers to learn optimal routing policies through interaction with the network environment, continually improving decisions based on feedback.

% \vspace{12pt}

% In large, dynamic networks where a central controller is impractical, decentralized execution is essential, making MARL crucial for enabling routers to operate independently. MARL systems empower routers to cooperate, compete, and coordinate their actions, achieving complex goals unattainable by a single controller. Therefore, introducing MARL has the potential to optimize network performance, improve adaptability to dynamic conditions, and ensure scalability as the network expands.

% \subsubsection{Decentralised Learning}

% Early approaches such as \textit{Q-routing} \cite{boyan1993packet} considered each router as an individual agent, applying Q-learning with a shared set of parameters for all routers. Each router maintains a Q-table that estimates the quality of routes to various destinations, updating these estimates based on observed packet delivery times to dynamically adjust to changing network conditions. Building upon Q-routing, \textit{DQN-routing} \cite{mukhutdinov2019multi} enhances this approach by integrating Deep Q-Networks (DQN) \cite{mnih2013playing}, leveraging deep learning to improve routing decisions and handle more complex network environments. 

% \subsubsection{Software Defined Networking}

% With the emergence of key technologies such as Software Defined Networking (SDN) \cite{shin2012software}, there has been a significant shift in how networks are managed. SDN decouples the control plane from the data plane, enabling more flexible and dynamic network management. In SDN, programmable switches are responsible for data forwarding, while a separate controller handles routing decisions. This separation contrasts with traditional networks, where routers have integrated control and data planes. The flexibility of SDN facilitates the application of networked MARL approaches by enabling routers and switches to communicate directly for control decisions.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/software_defined_network.png}
%     \caption{Comparison of Traditional Network and Software-Defined Network (SDN) architectures \cite{maleki2017sdn}.}
%     \label{fig:sdn}
% \end{figure}


% \subsubsection{Decentralized Learning with Networked Agents}

% SDN’s flexibility facilitates networked MARL approaches, enabling direct communication between routers and switches for control decisions. \textit{Deep Q-routing with Communication (DQRC)} \cite{you2020toward} enhances \textit{DQN-routing} by introducing a communication step between routers prior to action selection. Drawing from the success of \textit{Deep Recurrent Q-Network (DRQN)} \cite{hausknecht2015deep} in non-stationary settings, DQRC uses an LSTM layer to integrate local and neighboring observations, thereby improving adaptability and performance in dynamic network environments.

% \vspace{12pt}

% Conventional neural networks (feed-forward, recurrent, and convolutional) can specialize on specific graphs but struggle to generalize to unseen ones. In contrast, \textit{DRL+GNN} \cite{almasan2022deep} uses a Graph Neural Network (GNN) to process graph observations, allowing for generalization across different graph sizes and structures, making it a more robust solution for dynamic graphs. However, \textit{DRL+GNN} functions as a single-agent system with a central controller and full observability, where the GNN's effectiveness depends on the quality of the graph observations. This centralization, common in many modern methods \cite{casas2020intelligent, hope2021gddr, kim2022deep, schneider2021self}, limits scalability and reactivity compared to decentralized approaches.

% \vspace{12pt}

% To leverage GNNs in a decentralized multi-agent setting, the \textit{Graph-Query Neural Network} \cite{geyer2018learning} uses multiple communication rounds combined with a recurrent aggregation function \cite{li2015gated}. This approach allows agents to share observations and construct a global view of the environment. However, the decentralized nature introduces high non-stationarity, leading the authors to rely on supervised learning with labeled shortest path data. While this ensures stable training, it restricts agents to a single graph, limiting their ability to adapt and generalize to new graphs without retraining.

% \subsection{NetMon}

% The foundation of the proposed design is based on the NetMon architecture \footnote{While not explicitly mentioned in the paper, the name "NetMon" is used internally within the authors' code repository. For details, see \href{https://github.com/jw3il/graph-marl}{https://github.com/jw3il/graph-marl}.}, recently developed by Weil et al. \cite{weil2024towards}. NetMon has established itself as the leading framework for decentralized multi-agent reinforcement learning applied to network packet routing through a series of innovative contributions. This chapter provides the relevant background to understand some of the key advances which form the foundation of the proposed design.

% \subsubsection{Decoupling Node and Agent Observations}

% An intelligent router has two primary responsibilities: first, to build an internal representation of the network environment by storing experiences and communicating with neighboring routers; second, to use this representation to make optimal routing decisions. These tasks require different types of information and processing methods. For example, while packet-level data may be irrelevant for understanding the overall network, it is crucial for specific routing decisions. Similarly, GNNs are vital for learning environmental representations from graph-structured data, but a simpler DQN might suffice for making routing decisions.

% \addvspace{12pt}

% Previous MARL approaches treat this as a singular objective, requiring a single complex model to both process observations and make decisions. This demands significant computational resources and often restricts methods to centralized control or supervised learning, limiting flexibility and scalability.

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.64\linewidth]{figures/netmon-process-flow.png}
%     \caption{NetMon Process Flow \cite{weil2024towards}: Node models encode and share observations with neighboring nodes to update local states. These updated states are provided to agents for routing decisions.}
%     \label{fig:enter-label}
% \end{figure}

% Therefore, NetMon introduces a novel approach by decoupling the learning of graph observations from the process of making routing decisions. This separation provides a more flexible framework and addresses the primary cause of non-stationarity in networks—packet movement between routers—while the positions and availability of nodes remain relatively stationary during training. As a result, the learning of graph observations becomes nearly stationary, allowing decentralized nodes to develop effective graph representations without relying on supervised learning.

% \addvspace{12pt}

% \begin{algorithm}[H]
% \caption{Pseudo Offline Training for Decoupled Node and Agent Model}
% \label{alg:offline_graph_rl}
% \KwIn{Replay Memory $D$, Agent Model $Q$ with parameters $\theta_Q$, Node Model $U$ with parameters $\theta_U$, Learning rate $\alpha$}
% \For{each mini-batch $B$ from Replay Memory $D$}{
%     \For{each communication round $c$ in the sequence}{
%         \For{each agent $i$ in $B$}{
%             Update node state $h_v^i$ using the Node Model $U$ with parameters $\theta_U$\;
%         }
%     }
%     $L \gets 0$ \tcp{Initialize the mini-batch loss}
%     \For{each agent $i$ in $B$}{
%         Retrieve the local node state $h_v^i$ and observation $o^i$\;
%         Agent model predict Q-value $Q(h_v^i, o^i, a^i; \theta_Q)$\;
%         \tcp{Compute the mean squared TD error loss for sample $i$}
%         $y^i \gets r^i + \gamma \max_{a'} Q(h_{v+1}^i, s_{t+1}^i, a'; \theta_Q)$\;
%         $L_i \gets \left(Q(h_v^i, o^i, a^i; \theta_Q) - y^i \right)^2$\;
%         $L \gets L + L_i$ \tcp*{Accumulate $L_i$ into the mini-batch loss $L$}
%     }
%     \tcp{Backpropergate loss for both agent and node models}
%     $\theta_Q \gets \theta_Q - \alpha \nabla_{\theta_Q} L$\; 
%     $\theta_U \gets \theta_U - \alpha \nabla_{\theta_U} L$\;
% }
% \end{algorithm}

% To train the system end-to-end using reinforcement learning, the node model transfers its learned graph representation to the agent model whenever a packet arrives at a router. The agent then combines this graph representation with its local observations to make an informed routing decision. The resulting loss is backpropagated through both the node and agent models, allowing the entire system to refine its decision-making process and improve overall network performance. 


% \subsubsection{Multi-Round Recurrent Message Passing}

% In large distributed systems, effective graph representation learning hinges on efficient information propagation among agents. However, stacking convolutional layers often centralizes execution and introduces rigidity, as the fixed structure becomes a constraint during execution. A more flexible approach for fully decentralized and dynamic networks is multi-round recurrent communication \cite{weil2024towards, geyer2018learning}. This method allows agents to store and share relevant information across multiple communication rounds, ensuring that critical data is disseminated throughout the network. By eliminating the need for centralized control, this decentralized approach enables the system to adapt dynamically to changes in the network.

% \addvspace{12pt}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.9\linewidth]{figures/NetMon.png}
% \caption{\textit{NetMon} propagates information across the network through a recurrent message-passing model utilizing two LSTM networks to encode and aggregate information, respectively. \cite{weil2024towards}}
% \label{fig:netmon-reccurent-message}
% \end{figure}

% \addvspace{12pt}

% NetMon's bespoke recurrent message passing system uses two recurrent networks: one to encode and store local observations, and another to aggregate received messages from neighboring agents. The updated hidden representation is then sent to neighboring agents in the next communication round. Each node maintains its own local hidden state \(h^v\), which is zero-initialized after each environment step, and a cell state \(c^v\), which persists through communication rounds and environment steps.

% \addvspace{12pt}

% \begin{algorithm}[H]
% \caption{NetMon Distributed Node State Update}
% \label{alg:node_state_update}
% \KwIn{Node $v$ with direct neighbors $N(v)$, state $s$, previous node state $h^v$, node observation $m^v$, and $k$ communication rounds}
% $h^v_0 \gets \text{encode}(h^v, m^v)$ \tcp*{$\triangleright$ Encode node observation}
% \For{$k \gets 0$ to $K-1$} {
%     Send $h^v_k$ to all neighbors $w \in N(v)$\;
%     Receive $h^w_k$ from all neighbors $w \in N(v)$\;
%     $M^v_k \gets \text{aggregate}^k(\{h^w_k\}_{w \in N(v)})$\;
%     $h^v_{k+1} \gets \text{update}^k(h^v_k, M^v_k)$\tcp*{$\triangleright$ Update with message passing}
% }
% \textbf{return:} Updated node state $h^v_K$;
% \end{algorithm}

% \addvspace{12pt}

% Despite its simplicity, NetMon's custom recurrent message-passing system outperforms state-of-the-art models, delivering higher quality graph representations than both recurrent \cite{seo2018structured} and non-recurrent \cite{hamilton2017inductive, gravina2022anti} approaches.

% \subsubsection{Generalizable Pre-Training}

% Weil et al. pre-train their model across a diverse set of networks to ensure it is both generalizable and adaptable. This strategy mitigates the limitations of specialized models, such as susceptibility to local optima and the necessity for retraining when network conditions evolve. The pre-trained model can then be fine-tuned online during deployment, allowing for rapid adaptation to specific network conditions without the prohibitive costs and performance issues of training from scratch in a live environment. Crucially, by decoupling the node and agent observations the node environment becomes near stationary enabling NetMon to be trained end-to-end using reinforcement learning, setting it apart from earlier decentralized GNN methods that relied on supervised learning \cite{geyer2018learning}.

